Proactive Disentangled Modeling of Trigger-Object Pairings for Backdoor Defense

Deep neural networks (DNNs) and generative AI (GenAI) are increasingly vulnerable to backdoor attacks, where adversaries embed triggers into inputs to cause models to misclassify or misinterpret target labels. Beyond traditional single-trigger scenarios, attackers may inject multiple triggers across various object classes, forming unseen backdoor-object configurations that evade standard detection pipelines. In this paper, we introduce DBOM (Disentangled Backdoor-Object Modeling), a proactive framework that leverages structured disentanglement to identify and neutralize both seen and unseen backdoor threats at the dataset level. Specifically, DBOM factorizes input image representations by modeling triggers and objects as independent primitives in the embedding space through the use of Vision-Language Models (VLMs). By leveraging the frozen, pre-trained encoders of VLMs, our approach decomposes the latent representations into distinct components through a learnable visual prompt repository and prompt prefix tuning, ensuring that the relationships between triggers and objects are explicitly captured. To separate trigger and object representations in the visual prompt repository, we introduce the trigger-object separation and diversity losses that aids in disentangling trigger and object visual features. Next, by aligning image features with feature decomposition and fusion, as well as learned contextual prompt tokens in a shared multimodal space, DBOM enables zero-shot generalization to novel trigger-object pairings that were unseen during training, thereby offering deeper insights into adversarial attack patterns. Experimental results on CIFAR-10 and GTSRB demonstrate that DBOM robustly detects poisoned images prior to downstream training, significantly enhancing the security of DNN training pipelines.

==> Definitions/journalnames.tex <==
% Updated 18 December 2024 used for Y2025
%% --------------------------------------------------------------------
%\DeclareOption{}{%%
%		\gdef\@journal{}
%		\gdef\@journalfull{}
%		\gdef\@journalshort{}
%		\gdef\@doiabbr{}
%		\gdef\@ISSN{}
%		\gdef\@continuouspages{yes}
%		\gdef\@societyowner{}
%}
%% --------------------------------------------------------------------
%% Fields meanings:
%% - Option name: Journal website name (used in URL)
%% - @journal: Journal website name (used in URL)
%% - @journalshort: Short Name (ISO4)
%% - @journalfull: Journal full name
%% - @doiabbr: DOI abbreviation of the journal used in DOI numbers 10.32604/journalnameXXXX
%% - @ISSN: Journal E-ISSN number
%% - @continuouspages: use 	\gdef\@continuouspages{yes} for journals that use pagination
%% - @societyowner: Name of society owning the journal (for society journals)
%% --------------------------------------------------------------------
\DeclareOption{biocell}{%
	\gdef\@journal{biocell}
	\gdef\@journalshort{Biocell}
	\gdef\@journalfull{Biocell}
	\gdef\@doiabbr{biocell}
	\gdef\@ISSN{1667-5746}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{chd}{%
	\gdef\@journal{chd}
	\gdef\@journalshort{Congenit Heart Dis}
	\gdef\@journalfull{Congenital Heart Disease}
	\gdef\@doiabbr{chd}
	\gdef\@ISSN{1747-0803}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{cmc}{%
 	\gdef\@journal{cmc}
	\gdef\@journalshort{Comput Mater Contin.}
	\gdef\@journalfull{Computers, Materials \& Continua}
	\gdef\@doiabbr{cmc}	\gdef\@ISSN{1546-2226}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{cmes}{%
 	\gdef\@journal{cmes}
	\gdef\@journalshort{Comput Model Eng Sci}
	\gdef\@journalfull{Computer Modeling in Engineering \& Sciences}
	\gdef\@doiabbr{cmes}
	\gdef\@ISSN{1526-1506}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{csse}{%
 	\gdef\@journal{csse}
	\gdef\@journalshort{Comput Syst Sci Eng}
	\gdef\@journalfull{Computer Systems Science and Engineering}
	\gdef\@doiabbr{csse}
	\gdef\@ISSN{0267-6192}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}% ISSN (print)
\DeclareOption{dedt}{%
 	\gdef\@journal{dedt}
	\gdef\@journalshort{Digit Eng Digit Twin}
	\gdef\@journalfull{Digital Engineering and Digital Twin}
	\gdef\@doiabbr{dedt}
	\gdef\@ISSN{ }
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}% No ISSN
\DeclareOption{ee}{%
 	\gdef\@journal{ee}
	\gdef\@journalshort{Energy Eng}
	\gdef\@journalfull{Energy Engineering}
	\gdef\@doiabbr{ee}
	\gdef\@ISSN{1546-0118}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{fdmp}{%
 	\gdef\@journal{fdmp}
	\gdef\@journalshort{Fluid Dyn Mater Process}
	\gdef\@journalfull{Fluid Dynamics \& Materials Processing}
	\gdef\@doiabbr{fdmp}
	\gdef\@ISSN{1555-2578}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{fhmt}{%
 	\gdef\@journal{fhmt}
	\gdef\@journalshort{Front Heat Mass Transf}
	\gdef\@journalfull{Frontiers in Heat and Mass Transfer}
	\gdef\@doiabbr{fhmt}
	\gdef\@ISSN{2125-8629}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}% ISSN (print)
\DeclareOption{iasc}{%
 	\gdef\@journal{iasc}
	\gdef\@journalshort{Intell Autom Soft Comput}
	\gdef\@journalfull{Intelligent Automation \& Soft Computing}
	\gdef\@doiabbr{iasc}
	\gdef\@ISSN{2326-005X}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{icces}{%
 	\gdef\@journal{icces}
	\gdef\@journalshort{Int Conf Comput Exp Eng Sci}
	\gdef\@journalfull{The International Conference on Computational \& Experimental Engineering and Sciences}
	\gdef\@doiabbr{icces}
	\gdef\@ISSN{1993-2815}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{ijmhp}{%
 	\gdef\@journal{ijmhp}
	\gdef\@journalshort{Int J Ment Health Promot}
	\gdef\@journalfull{International Journal of Mental Health Promotion}
	\gdef\@doiabbr{ijmhp}
	\gdef\@ISSN{2049-8543}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{jai}{%
 	\gdef\@journal{jai}
	\gdef\@journalshort{J Artif Intell}
	\gdef\@journalfull{Journal on Artificial Intelligence}
	\gdef\@doiabbr{jai}
	\gdef\@ISSN{2579-003X}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{jbd}{%
 	\gdef\@journal{jbd}
	\gdef\@journalshort{J Big Data}
	\gdef\@journalfull{Journal on Big Data}
	\gdef\@doiabbr{jbd}
	\gdef\@ISSN{2579-0056}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{jbic}{%
 	\gdef\@journal{jbic}
	\gdef\@journalshort{J Blockchain Intell Comput}
	\gdef\@journalfull{Journal of Blockchain and Intelligent Computing}
	\gdef\@doiabbr{jbic}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}% No ISSN
\DeclareOption{jcs}{%
 	\gdef\@journal{jcs}
	\gdef\@journalshort{J Cyber Secur}
	\gdef\@journalfull{Journal of Cyber Security}
	\gdef\@doiabbr{jcs}
	\gdef\@ISSN{2579-0064}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{jihpp}{%
 	\gdef\@journal{jihpp}
	\gdef\@journalshort{J Inf Hiding Priv Prot}
	\gdef\@journalfull{Journal of Information Hiding and Privacy Protection}
	\gdef\@doiabbr{jihpp}
	\gdef\@ISSN{2637-4226}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{jimh}{%
 	\gdef\@journal{jimh}
	\gdef\@journalshort{JIMH}
	\gdef\@journalfull{Journal of Intelligent Medicine and Healthcare}
	\gdef\@doiabbr{jimh}
	\gdef\@ISSN{2837-634X}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{jiot}{%
 	\gdef\@journal{jiot}
	\gdef\@journalshort{J Internet Things}
	\gdef\@journalfull{Journal on Internet of Things}
	\gdef\@doiabbr{jiot}
	\gdef\@ISSN{2579-0080}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{jnm}{%
 	\gdef\@journal{jnm}
	\gdef\@journalshort{J New Media}
	\gdef\@journalfull{Journal of New Media}
	\gdef\@doiabbr{jnm}
	\gdef\@ISSN{2579-0129}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{jpm}{%
 	\gdef\@journal{jpm}
	\gdef\@journalshort{J Polym Mater}
	\gdef\@journalfull{Journal of Polymer Materials}
	\gdef\@doiabbr{jpm}
	\gdef\@ISSN{0976-3449}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{jqc}{%
 	\gdef\@journal{jqc}
	\gdef\@journalshort{J Quantum Comput}
	\gdef\@journalfull{Journal of Quantum Computing}
	\gdef\@doiabbr{jqc}
	\gdef\@ISSN{2579-0145}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{jrm}{%
 	\gdef\@journal{jrm}
	\gdef\@journalshort{J Renew Mater}
	\gdef\@journalfull{Journal of Renewable Materials}
	\gdef\@doiabbr{jrm}
	\gdef\@ISSN{2164-6341}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{or}{%
 	\gdef\@journal{or}
	\gdef\@journalshort{Oncol Res}
	\gdef\@journalfull{Oncology Research}
	\gdef\@doiabbr{or}
	\gdef\@ISSN{1555-3906}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{phyton}{%
 	\gdef\@journal{phyton}
	\gdef\@journalshort{Phyton-Int J Exp Bot}
	\gdef\@journalfull{Phyton-International Journal of Experimental Botany}
	\gdef\@doiabbr{phyton}
	\gdef\@ISSN{1851-5657}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{po}{%
 	\gdef\@journal{po}
	\gdef\@journalshort{Psycho-Oncologie}
	\gdef\@journalfull{Psycho-Oncologie}
	\gdef\@doiabbr{po}
	\gdef\@ISSN{1778-381X}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{rig}{%
 	\gdef\@journal{rig}
	\gdef\@journalshort{Rev Int Géomatique}
	\gdef\@journalfull{Revue Internationale de Géomatique}
	\gdef\@doiabbr{rig}
	\gdef\@ISSN{2116-7060}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{sdhm}{%
 	\gdef\@journal{sdhm}
	\gdef\@journalshort{Struct Durab Health Monit}
	\gdef\@journalfull{Structural Durability \& Health Monitoring}
	\gdef\@doiabbr{sdhm}
	\gdef\@ISSN{1930-2991}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{sv}{%
 	\gdef\@journal{sv}
	\gdef\@journalshort{Sound Vib}
	\gdef\@journalfull{Sound \& Vibration}
	\gdef\@doiabbr{sv}
	\gdef\@ISSN{2693-1443}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{notspecified}{%
	\gdef\@journal{notspecified}
	\gdef\@journalfull{Journal Not Specified}
	\gdef\@journalshort{Journal Not Specified}
	\gdef\@doiabbr{journal}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
}
\DeclareOption{test}{%
	\gdef\@journal{test}
	\gdef\@journalfull{TEST}
	\gdef\@journalshort{TEST}
	\gdef\@doiabbr{test}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
}
